Multi-modal Pose Diffuser: A Multimodal Generative Conditional Pose Prior

The Skinned Multi-Person Linear (SMPL) model plays a crucial role in 3D human pose estimation, providing a streamlined yet effective representation of the human body. However, ensuring the validity of SMPL configurations during tasks such as human mesh regression remains a significant challenge , highlighting the necessity for a robust human pose prior capable of discerning realistic human poses. To address this, we introduce MOPED: \underline{M}ulti-m\underline{O}dal \underline{P}os\underline{E} \underline{D}iffuser. MOPED is the first method to leverage a novel multi-modal conditional diffusion model as a prior for SMPL pose parameters. Our method offers powerful unconditional pose generation with the ability to condition on multi-modal inputs such as images and text. This capability enhances the applicability of our approach by incorporating additional context often overlooked in traditional pose priors. Extensive experiments across three distinct tasks-pose estimation, pose denoising, and pose completion-demonstrate that our multi-modal diffusion model-based prior significantly outperforms existing methods. These results indicate that our model captures a broader spectrum of plausible human poses.

==> sections/figures/denoising.tex <==
\begin{table}[!t]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{lcc}
\toprule
\textbf{Method}                     & $\Delta\textbf{q}+\text{m2m}\downarrow$ & $\text{m2m}(\text{cm})\downarrow$   \\
\midrule
PoseNDF\cite{tiwari2022pose}    & - & - \\
NRDF\cite{he2024nrdf}           & 0.313 & 24.93 \\
DPoser\cite{lu2023dposer}          & - & - \\
% \method{} (Ours, $t=1000, \Delta 5$)                & 0.093 & 8.58 \\
% \method{} (Ours, $t=900, \Delta 5$)                & 0.301 & 23.60 \\
\method{} (Ours, $t=900, \Delta 5$)                & 0.322 & 24.93 \\
% \method{} (Ours, $t=900, \Delta 10$)                & 0.075 & 7.01 \\
% \method{} (Ours, $t=900, \Delta 5$)                & 0.084 & 7.84 \\
% \method{} (Ours, $t=900, \Delta 2$)                & 0.109 & 9.95 \\
% \method{} (Ours, $t=400, \Delta 5$)                & 0.133 & 11.72 \\
% \method{} (Ours, $t=400, \Delta 2$)               & 0.146 & 12.81\\
% \method{} (Ours, $t=200, \Delta 2$)               & 0.207 & 17.05\\
\bottomrule
\end{tabular}
\label{Table:denoise}
\caption{TODO:regenerate noisy poses. Comparison with baseline methods for pose denoising. m2m is reported in centimeters. Testing other choices in time-steps scheduling show that choosing the right start step is critical. Consistency models\cite{song2023consistency} and other alternatives may be able to help remove the need to choose the optimal parameters.} 
\end{table}

==> sections/figures/hmr_different_datasets.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[picture format/.style={inner sep=3pt, outer sep=1pt}]

  \node[picture format]                   (A1)               {\includegraphics[trim=350 0 350 0,clip, width=1.15in]{sections/figures/hmr_images/ours/01_img_[82.61552066640219]_[128.095022308605]mesh_fit.png}};
  \node[picture format,anchor=north]      (B1) at (A1.south) {\includegraphics[trim=350 0 350 0,clip, width=1.15in]{sections/figures/hmr_images/ours/05_img_[68.96444262276147]_[76.62396137146361]mesh_fit.png}};
\node[picture format,anchor=north]      (C1) at (B1.south) {\includegraphics[trim=350 0 350 0,clip, width=1.15in]{sections/figures/hmr_images/ours/09_img_[53.447338233828674]_[71.96820752530422]mesh_fit.png}};
  \node[picture format,anchor=north]      (D1) at (C1.south) {\includegraphics[trim=350 0 350 0,clip, width=1.15in]{sections/figures/hmr_images/ours/18_img_[74.1666871091886]_[121.5710905741555]mesh_fit.png}};


  \node[picture format,anchor=north west] (A2) at (A1.north east) {\includegraphics[trim=300 450 200 300,clip, width=.9in]{sections/figures/hmr_images/3dpw/image_00210_mesh_fit.png}};
  \node[picture format,anchor=north]      (B2) at (A2.south)      {\includegraphics[trim=225 10 850 10,clip, width=.9in]{sections/figures/hmr_images/3dpw/image_00325_mesh_fit.png}};
    \node[picture format,anchor=north]      (C2) at (B2.south)      {\includegraphics[trim=140 200 500 250,clip, width=.4in]{sections/figures/hmr_images/3dpw/image_01297.png}};
      \node[picture format,anchor=north]      (D2) at (C2.south)      {\includegraphics[trim=350 10 950 10,clip,width=.9in]{sections/figures/hmr_images/3dpw/image_01108_mesh_fit.png}};

  \node[picture format,anchor=north west] (A3) at (A2.north east) {\includegraphics[trim=140 50 400 60,clip,width=.60in]{sections/figures/hmr_images/coco/COCO_train2014_000000031335_mesh_fit.png}};
  \node[picture format,anchor=north]      (B3) at (A3.south)      {\includegraphics[trim=0 90 200 100,clip,width=.75in]{sections/figures/hmr_images/coco/COCO_train2014_000000273665_mesh_fit.png}};
    \node[picture format,anchor=north]      (C3) at (B3.south)      {\includegraphics[trim=400 0 0 0,clip,width=.65in]{sections/figures/hmr_images/coco/COCO_train2014_000000175669_mesh_fit.png}};
      \node[picture format,anchor=north]      (D3) at (C3.south)      {\includegraphics[trim=100 100 400 100,clip,width=0.7in]{sections/figures/hmr_images/coco/COCO_train2014_000000525169_mesh_fit.png}};

  %% Captions

  \node[anchor=south] (E1) at (A1.north) {\bfseries EHF};
  \node[anchor=south] (E2) at (A2.north) {\bfseries 3DPW\cite{vonMarcard2018}};
  \node[anchor=south] (E3) at (A3.north) {\bfseries COCO\cite{lin2014microsoft}};

\end{tikzpicture}
\caption{Qualitative Results from \method{} for 3D pose estimation across the EHF\cite{SMPL-X:2019}, 3DPW\cite{vonMarcard2018}, and COCO\cite{lin2014microsoft} show that our model can perform well in a wide range of scenarios. The poses are over-layed over the original images which are available in the Supplementary Material.} 
\label{fig:qual_hmr}
\end{figure}

==> sections/figures/hmr_examples.tex <==
\begin{figure*}[t!]
\centering
\begin{tikzpicture}[picture format/.style={inner sep=5pt,}]


  % \node[picture format]                   (A1)               {\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/ours/ehf_gt/01_img.png}};
    \node[picture format]                   (A1)              {\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/ours/ehf_gt/05_img.png}};
    % \node[picture format,anchor=north]      (C1) at (B1.south) {\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/ours/ehf_gt/09_img.png}};

  % \node[picture format, anchor=north west] (A2) at (A1.north east){\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/ours/01_img_[82.61552066640219]_[128.095022308605]mesh_fit.png}};
  \node[picture format,anchor=north west]      (A2) at (A1.north east) {\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/ours/05_img_[68.96444262276147]_[76.62396137146361]mesh_fit.png}};
    % \node[picture format,anchor=north]      (C2) at (B2.south) {\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/ours/09_img_[53.447338233828674]_[71.96820752530422]mesh_fit.png}};

  % \node[picture format,anchor=north west] (A3) at (A2.north east) {\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/dposer/01_img_mesh_fit.png}};
  \node[picture format,anchor=north west]      (A3) at (A2.north east)      {\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/dposer/05_img_mesh_fit.png}};
    % \node[picture format,anchor=north]      (C3) at (B3.south)      {\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/dposer/09_img_mesh_fit.png}};

  % \node[picture format,anchor=north west] (A4) at (A3.north east) {\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/posendf/01_img_[210.20784889717345]_[267.5707375239675]_mesh_fit.png}};
  \node[picture format,anchor=north west]      (A4) at (A3.north east)      {\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/posendf/05_img_[151.21564345207153]_[277.34793353709813]_mesh_fit.png}};
    % \node[picture format,anchor=north]      (C4) at (B4.south)      {\includegraphics[trim=350 0 350 0,clip, width=1.0in]{sections/figures/hmr_images/posendf/09_img_[74.66004911795598]_[151.95715054949346]_mesh_fit.png}};

  %% Captions
 \node[anchor=south] (D1) at (A1.north) {\bfseries Original};
\node[anchor=south] (D2) at (A2.north) {\bfseries \method{} (Ours)};
  \node[anchor=south] (D3) at (A3.north) {\bfseries DPoser};
  \node[anchor=south] (D4) at (A4.north) {\bfseries PoseNDF};

\end{tikzpicture}


\caption{Qualitative Results on the EHF \cite{SMPL-X:2019} dataset. Visually both DPoser \cite{lu2023dposer} and PoseNDF \cite{tiwari2022pose} estimate poses that are physically not possible for a human. In the top row we see the subjects right shoulder is in an impossible position. In the second row the subjects arms are both in front of them but DPoser\cite{lu2023dposer} and and PoseNDF \cite{tiwari2022pose} make the mistake of pushing the arms to be behind the person. In the third row we see that our model avoids self-intersections while both DPoser \cite{lu2023dposer} and PoseNDF \cite{tiwari2022pose} fail to do so. Larger images can be found in the Supplementary Material. \amit{This figure is probably incomplete as there are no rows. Put in more images like other papers. Cite the figure in the text and explain.}
}
\label{fig:ehf}
\end{figure*}

==> sections/figures/motion_denoising.tex <==
% \begin{table}[]
% \centering
% \setlength{\tabcolsep}{12pt}
% \caption{We demonstrate the effectiveness of our prior on the motion denoising task.}
% \begin{tabular}{llll}
% \toprule
%               \multirow{2}{}{\textbf{Algorithm}}                                 &                                & \multicolumn{1}{c}{\textbf{MPJPE}}       &                                 \\
% \cmidrule{2-4}
%                         & $\sigma=20$& $\sigma=40$&$\sigma=100$ \\ 
% \midrule
% VPoser\cite{SMPL-X:2019}      & \multicolumn{1}{c}{-}  & 23.42           & \multicolumn{1}{c}{-}  \\
% Pose-NDF\cite{tiwari2022pose} & \multicolumn{1}{c}{-}  & 26.80           & \multicolumn{1}{c}{-}  \\
% HuMoR\cite{rempe2021humor}    & \multicolumn{1}{c}{-}  & 22.69           & \multicolumn{1}{c}{-} \\
% DPoser\cite{lu2023dposer}     & 13.64                  & 19.87           & 33.18                 \\
% \method{}(Ours)                          & \textbf{09.23}          &\textbf{14.63}  & \textbf{28.95} \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}
% \centering
% % \setlength{\tabcolsep}{12pt}
% \caption{We demonstrate the effectiveness of our prior on the motion denoising task. Specifically, we are focused on the $\sigma=40$ noise level and compare against existing methods on those settings in terms of MPJPE with numbers as reported in DPoser\cite{lu2023dposer}. Furthermore, we compare against DPoser\cite{lu2023dposer}, the most recent state of the art pose prior. Additional noise level results are available in the Appendix}
% \begin{tabular}{cc}
% \toprule
% % \multirow{2}{*}{\textbf{Algorithm}} & & \multicolumn{1}{c}{\textbf{MPJPE}} & \\
% \textbf{Method} & \textbf{MPJPE}
% % \cmidrule{2-4}
% % & $\sigma=20$& $\sigma=40$&$\sigma=100$ \\
% \midrule
% VPoser\cite{SMPL-X:2019} &  23.42  \\
% Pose-NDF\cite{tiwari2022pose} &  26.80 \\
% HuMoR\cite{rempe2021humor} &  22.69  \\
% DPoser\cite{lu2023dposer} & 19.87 \\
% \method{}(Ours) & \textbf{14.63} \\
% \bottomrule
% \label{table: denoise}
% \end{tabular}
% \end{table}    




\begin{table}[t!]
    \centering
    \caption{Here we demonstrate that \method{} offers superior performance for pose estimation when compared to other priors and refinement methods. (CLIFF) denotes that the prior was initialized by the output of CLIFF\cite{li2022cliff}. Even with a strong initialization we are still beating prior works.}
    % \setlength{\tabcolsep}{10pt}
    \begin{tabular}{cc}
    \toprule
    \textbf{Method}   & \textbf{MPJPE} & \\
    \midrule
VPoser\cite{SMPL-X:2019} &  23.42  \\
Pose-NDF\cite{tiwari2022pose} &  26.80 \\
HuMoR\cite{rempe2021humor} &  22.69  \\
DPoser\cite{lu2023dposer} & 19.87 \\
\method{}(Ours) & \textbf{14.63} \\
    \bottomrule
    \end{tabular}
    \label{table:hmr}
\end{table}


    
    % \begin{table}[]
    %     \centering
    %     \begin{tabular}{ll}
    %     Method                          & MPJPE   \\
    %     \hline
    %     VPoser                          & 23.42    \\
    %     Pose-NDF\cite{tiwari2022pose}   & 26.80    \\
    %     DPoser                          & 19.87     \\
    %     Ours                            & \textbf{14.63} 
    %     \end{tabular}
    %     \caption{We demonstrate the effectiveness of our prior on the motion denoising task.}
    % \end{table}
